A Concurrency-Optimal Binary Search Tree

The paper presents the first \emph{concurrency-optimal} implementation of a binary search tree (BST). The implementation, based on a standard sequential implementation of an internal tree, ensures that every \emph{schedule} is accepted, i.e., interleaving of steps of the sequential code, unless linearizability is violated. To ensure this property, we use a novel read-write locking scheme that protects tree \emph{edges} in addition to nodes. Our implementation outperforms the state-of-the art BSTs on most basic workloads, which suggests that optimizing the set of accepted schedules of the sequential code can be an adequate design principle for efficient concurrent data structures.

==> conc.tex <==
\begin{algorithm*}[t]
\caption{Concurrent implementation of binary search tree.}
\label{alg:concur}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\scriptsize
	
	\Part{Shared variables}{
		\State node is a record with fields: 
		\State $\ms{val}$, its value
		\State $\ms{left}$, its pointer to the left child in the tree
		\State $\ms{deleted}$, a boolean indicating logical deleted
		\State $\ms{vlock}$, a versioned lock: counter whose least significant bit is a lock
		\State Initially the tree contains one node $\ms{root}$,
		\State $\ms{root.val} = +\infty$
		\State $\ms{root.deleted} = true$
		\State $\ms{root.vlock} = \langle 0, false \rangle$
	}\EndPart
	
	\Statex
	
	
	\Part{$\lit{validate(\ms{gprev}, \ms{prev}, \ms{curr})}$}{
		\If{$\ms{gprev} \ne null$}
			\State $\ms{gpVer} \gets \ms{gprev.vlock.getVersion()}$ \Comment{return lock-version}
			\If{$\ms{prev}$ is not child of $\ms{gprev}$}
				\Return $\bot$ \EndReturn
			\EndIf
		\EndIf
		\State $\ms{pVer} \gets \ms{prev.vlock.getVersion()}$ \Comment{return lock-version}
		
		\If{$\ms{curr}$ is not child of $\ms{prev}$}
			\Return $\bot$ \EndReturn
		\EndIf
		
		\Return $\langle \ms{gpVer}, \ms{pVer} \rangle$ \EndReturn
	}\EndPart

	\Statex
	
	\Part{$\lit{insert}(v)$}{
		\State $\ms{prev}, \ms{curr} \gets traversal(v)$
		\If{$\langle gpVer, pVer \rangle \gets validate(null, gprev, prev) = \bot$}
			\State goto line 20 \Comment{abort: restart from the beginning}
		\EndIf
	
		\If{$\ms{curr} \ne null$} \Comment{first case}
			%\If{$\lnot \ms{curr.deleted}$}
			%	\Return \false \EndReturn \Comment{vertex is already in the set}
			%\EndIf
			
			\If{$\lnot \ms{prev.vlock.tryLockAtVersion(pVer)}$}
				\State goto Line 20 \Comment{abort}
			\EndIf
			
			\State $\ms{curr.lockAtCurrentVersion()}$ \Comment{spin lock}
			\State $\ms{ret} = curr.deleted$ \Comment{save the result}
			\If{$\ms{ret}$} $\ms{curr.deleted} = \false$ \EndIf
			\State $\ms{curr.vlock.unlockAndIncrementVersion()}$
			\State $\ms{prev.vlock.unlockAndIncrementVersion()}$
		\Else \Comment{second case}
			\State $\ms{newNode.val} \gets v$ \Comment{allocate a new node with value v}
			
			\If{$\lnot \ms{prev.vlock.tryLockAtVersion(pVer)}$}
			%	\State $\ms{gprev.vlock.unlock()}$
				\State goto Line 20 \Comment{abort}
			\EndIf
			
			\If{$v < \ms{prev.val}$}
				\State $\ms{prev.left} \gets newNode$
			\Else
				\State $\ms{prev.right} \gets newNode$
			\EndIf
			
			\State $\ms{prev.vlock.unlockAndIncrementVersion()}$
			\State $\ms{ret} = \true$
		\EndIf
		
		\Return $\ms{ret}$ \EndReturn
   	}\EndPart
	
	\Statex
	
	\Part{$\lit{delete}(v)$}{
		\State $\ms{gprev}, \ms{prev}, \ms{curr} \gets traversal(v)$
		\If{$\langle gpVer, pVer \rangle \gets validate(gprev, prev, curr) = \bot$}
			\State goto line 44 \Comment{abort: restart from the beginning}
		\EndIf
		
		\If{$\ms{curr.val} \ne v \lor \ms{curr.deleted}$}
			\Return \false \EndReturn \Comment{v is not in the set}
		\EndIf
		
		\If{$\lnot \ms{gprev.vlock.tryLockAtVersion(gpVer)}$}
			\State goto Line 44 \Comment{abort}
		\EndIf
			
		\If{$\lnot \ms{prev.vlock.tryLockAtVersion(pVer)}$}
			\State $\ms{gprev.vlock.unlock()}$
			\State goto Line 44 \Comment{abort}
		\EndIf
		
		\State $\ms{curr.lockAtCurrentVersion()}$ \Comment{spin lock}
		\If{$\ms{curr}$ has 2 children} \Comment{case 1}
			\State $\ms{curr.deleted} \gets \true$
		\EndIf
		
		\If{$\ms{curr}$ has 1 child}
			\If{$\ms{curr.left} \ne null$}
				$\ms{child} \gets \ms{curr.left}$
			\Else
				$~\ms{child} \gets \ms{curr.left}$
			\EndIf
			
			\If{$\ms{child.val} < \ms{curr.val}$}
				$\ms{prev.left} \gets \ms{child}$
			\Else
				$~\ms{prev.right} \gets \ms{child}$
			\EndIf
		\EndIf
		
		\If{$\ms{curr}$ is a leaf} \Comment{case 3}
			\If{$\ms{prev.deleted}$} \Comment{case 3, second subcase}
				\State \Comment{save second child of $\ms{prev}$ into $\ms{child}$}
				\If{$\ms{curr}$ is left child of $\ms{prev}$} 
					$\ms{child} \gets \ms{prev.right}$
				\Else
					$~\ms{child} \gets \ms{prev.left}$
				\EndIf
				
				\If{$\ms{prev}$ is left child of $\ms{gprev}$}
					$\ms{gprev.left} \gets child$
				\Else
					$~\ms{gprev.right} \gets child$
				\EndIf
			\Else \Comment{case 3, second subcase}
				\If{$\ms{curr}$ is left child of $\ms{prev}$}
					$\ms{prev.left} \gets null$
				\Else
					$~\ms{prev.right} \gets null$
				\EndIf
			\EndIf
		\EndIf
		
		\State $\ms{gprev.vlock.unlockAndIncrementVersion()}$
		\State $\ms{prev.vlock.unlockAndIncrementVersion()}$
		\State $\ms{curr.vlock.unlockAndIncrementVersion()}$
		
		\Return \true \EndReturn
   	}\EndPart
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}

%


==> figure2.tex <==
\begin{tikzpicture}
\node (r1) at (1,0) [] {};
%\node (r2) at (3,0) [] {};
\node (r3) at (3,0) [] {};
%\node (r4) at (7,0) [] {};
\node (w1) at (5,0) [] {};

\node (r11) at (2,-1) [] {};
%\node (r21) at (4,-1) [] {};
\node (r31) at (4,-1) [] {};
\node (r41) at (7,-1) [] {};



\draw  (1,0)  [black,fill=black, radius=0.1] circle (0.5ex);
%\draw  (3,0)  [black,fill=black, radius=0.1] circle (0.5ex);
\draw  (3,0)  [black,fill=black, radius=0.1] circle (0.5ex);
%\draw  (7,0)  [black,fill=black, radius=0.1] circle (0.5ex);
\draw  (4,0)  [black,fill=black, radius=0.1] circle (0.5ex);

\draw (r1) node [above] {\large {$R(r)$}};
%\draw (r2) node [above] {\small {$R(H)$}};
\draw (r3) node [above] {\large {$R(X_2)$}};
%\draw (r4) node [above] {\small {$R(X_1)$}};
\draw (w1) node [above] {\large {$\ms{new}(X_2)$}};

\draw  (2,-1)  [black,fill=black, radius=0.1] circle (0.5ex);
%\draw  (4,-1)  [black,fill=black, radius=0.1] circle (0.5ex);
\draw  (5,-1)  [black,fill=black, radius=0.1] circle (0.5ex);
%\draw  (12,-1)  [black,fill=black, radius=0.1] circle (0.5ex);
\draw  (7,-1)  [black,fill=black, radius=0.1] circle (0.5ex);

\draw (r11) node [above] {\large {$R(r)$}};
%\draw (r21) node [above] {\small {$R(H)$}};
\draw (r31) node [above] {\large {$R(X_2)$}};
\draw (r41) node [above] {\large {$\ms{new}(X_3)$}};

\begin{scope}   
\draw [|-|,thick] (0,0) node[left] {\large $\lit{insert}(1)$} to (6,0) node[right] {\large $\true$};
\draw [|-|,thick] (1,-1) node[left] {\large $\lit{insert}(3)$} to (8,-1) node[right] {\large $\true$};
% \draw [-, dotted] (8,-1) to (8,1) node[right] {\large $E'$};
% \draw [-, dotted] (9,-1) to (9,1) node[right] {\large $E$};
\end{scope}
\node[draw,align=left] at (-2,-.5) {\large \{2\}};
% \node[draw,align=left] at (7.8,-2.1) {{\large $\lit{insert}(1)$ must acquire}\\{\large the lock on $X_1$ prior to}\\{\large returning $\false$ in $E$}};
% \node[draw,align=left] at (8,1.8) {{\large $\lit{insert}(2)$ holds the}\\{\large lock on $X_1$ after $E'$}};

%
\end{tikzpicture}


==> linearization.tex <==
\section{Correctness}
\label{ch:correctness}
\subsection{Preliminaries}
\textbf{Objects and implementations.}
We consider a standard asynchronous shared-memory system, in which $n > 1$ processes $p_1, \dots, p_n$ 
communicate by applying operations on shared \textit{objects}. An object is an instance of
an \textit{abstract data type} that specifies the set of operations the object exports, the set of responses the operations
return, the set of states the object can take, and the sequential specification that stipulates the object’s correct
sequential behaviour. To \textit{implement} a \textit{high-level} object from a set of shared \textit{base} objects, 
processes follow an algorithm, which is a collection of deterministic state machines, one for each process. The algorithm assigns
initial values to the base objects and processes and specifies the base-object operations a process must perform
when it executes every given operation. To avoid confusion, we call operations on the base objects \textit{primitives}.
A primitive is an atomic \textit{read-modify-write (rmw)} on a base object characterized by a pair of deterministic
functions $\langle g, h\rangle$: given the current state of the base object, $g$ is an \textit{update} function 
that computes its state after the primitive is applied, while $h$ is a \textit{response} function that specifies 
the outcome of the primitive returned to the process. Special cases of rmw primitives are 
\textit{read} ($g$ leaves the state unchanged and $h$ returns the state) and 
\textit{write} ($g$ updates the state with its argument and $h$ returns ok).

\textbf{Executions}
An \textit{event} of a process $p_i$ is an invocation or response of an operation performed by $pi$ on a highlevel
object implementation, a rmw primitive $\langle h, g \rangle$, applied by $p_i$ to a base object $b$ along with its response $r$
(we call it a \textit{rmw event} and write $(b, \langle g, h \rangle, r, i)$). 
A \textit{configuration} specifies the value of each base object and the state of each process. 
The \textit{initial configuration} is the configuration in which all base objects have their initial
values and all processes are in their initial states.

An \textit{execution fragment} is a (finite or infinite) sequence of events. An \textit{execution} of an implementation $I$ is an
execution fragment where, starting from the initial configuration, each event is issued according to $I$ and each response of a rmw event $(b, \langle g, h \rangle, r, i)$ matches the state of $b$ resulting from all preceding events. 
We assume that executions are \textit{well-formed}: no process invokes a new high-level operation before the previous high-level
operation returns.

Let $\alpha \mid p_i$ denote the subsequence of an execution $\alpha$ restricted to the events of process $p_i$.
Executions $\alpha$ and $\alpha'$ are \textit{equivalent} if for every process $p_i$, $\alpha \mid p_i = \alpha' \mid p_i$.
An operation $\pi$ \textit{precedes} another operation $\pi'$ in an execution $\alpha$, denoted $\pi \to_{\alpha} \pi'$, 
if the response of $\pi$ occurs before the invocation of $\pi'$ in $\alpha$. 
Two operations are \textit{concurrent} if neither precedes the other. 
An execution is \textit{sequential} if it has no concurrent operations. 
An operation is \textit{complete} in $\alpha$ if the invocation event is followed by a \textit{matching} response; 
otherwise, it is incomplete in $\alpha$. 
Execution $\alpha$ is complete if every operation is complete in $\alpha$.

\subsection{Safety. Linearizability.}
\textbf{High-level histories and linearizability.}
A \textit{high-level history} $\widetilde{H}$ of an execution $\alpha$ is the subsequence of $\alpha$
consisting of all invocations and responses of (high-level) operations.

A complete high-level history $\widetilde{H}$ is \textit{linearizable} with respect to an object type $\tau$ 
if there exists a sequential high-level history $S$ equivalent to $\widetilde{H}$ such that 
\begin{enumerate}
  \item $\to_{\widetilde{H}} \subseteq \to_S$
  \item $S$ is consistent with the sequential specification of type $\tau$.
\end{enumerate}

Now a high-level history $\widetilde{H}$ is linearizable if it can be \textit{completed} (by adding matching responses to a subset
of incomplete operations in $\widetilde{H}$ and removing the rest) to a linearizable high-level history.

\textbf{Sequential implementations.}
A \textit{sequential implementation} of an object type $\tau$ specifies, for each operation of $\tau$, a deterministic 
procedure that performs \textit{read} and \textit{write} primitives on a collection of base objects that encode the state 
of the object, and returns a response, so that the specification of $\tau$ is respected in all sequential executions.

Consider the conventional \textbf{set} type exporting $\lit{insert}$, \textbf{remove}, and $\lit{contains}$ operations 
with standard sequential semantics: $\lit{insert}(v)$ adds $v$ to the set and returns $\true$ if $v$ is not already there, 
and returns $\false$ otherwise;
$\textbf{remove}(v)$ drops $v$ from the set and returns $\true$ if $v$ is there, and returns $\false$ otherwise; 
and $\lit{contains}(v)$ returns $\true$ if and only if $v$ is in the set. 
The exact specification and the tree-based sequential implementation of set are presented in Algorithm~\ref{alg:seq}.

\subsection{Proof of linearizability of Binary Search Tree}
\textbf{Linearization points.} Let $\alpha$ be a finite execution of the algorithm and $<_{\alpha}$ denote the total order
of events on $\alpha$. For the sake of the proof, we assume that $\alpha$ starts with an artificial sequential
execution of an insert operation $\pi_0$ that inserts root with key $+\infty$. Let $H$ be the high-level history exported by $\alpha$.

To prove linearizability of our algorithm, we need to define the linearization points of
insert, delete and contains operations.

\textit{Completions.} We obtain a completion $\tilde{H}$ of $H$ as follows. The invocation of an incomplete
contains operation is discarded. The invocation of an incomplete $\pi = delete$ operation that has
not performed a write at Lines 15, 25, 40 (43), 56 (60) of the Algorithm~\ref{alg:concur-del} is discarded;
otherwise, it is completed with the response true. The invocations of an incomplete $\pi = insert$
operation that has not performed a write at Lines 16, 23 (25) of the Algorithm~\ref{alg:concur-ins} are
discarded; otherwise, $\pi$ is completed with the response $\true$.

\textit{Linearization points.} We obtain a sequential high-level history $\tilde{S}$ equivalent to $\tilde{H}$ 
by associating a linearization point $l_{\pi}$ with each operation $\pi$.
In some cases, our choice of the linearization point of $\pi$ depends on the time interval between the start time and the end time of
 the execution of $\pi$, later referred to as the interval of $\pi$. 
For example, the linearization point of $\pi$ in the timeline should lie in the range of $\pi$.

Now we could specify the linearization points of the operation $\pi$ depending on its type.

\textbf{Insert.}
For every $\pi = insert(v)$ that returns $\true$, we have two cases:
\begin{enumerate}
\item A vertex with key $v$ was found in the tree. T
hen $l_{\pi}$ is associated with the write in Line 16
\item A vertex with key $v$ was not found in the tree. 
Then $l_{\pi}$ is associated with the writes in Lines 23 or 25, depending on whether the inserted vertex is left or right child.
\end{enumerate}
For every $\pi = insert(v)$ that returns $\false$, $l_{\pi}$ is associated with the last read in Line 10.

\textbf{Delete.}
For every $\pi = delete(v)$ that returns $\true$ we have four cases, 
depending on the number of children of the vertex with key $v$, i.e. the vertex $\ms{curr}$:
\begin{enumerate}
\item $\ms{curr}$ has two children. Then $l_{\pi}$ is associated with the write in Line 15.
\item $\ms{curr}$ has one child. Then $l_{\pi}$ is associated with the write in Lines 27 or 31, 
depending on whether $\ms{curr}$ is left or right child.
\item $\ms{curr}$ is a leaf with a DATA parent. Then $l_{\pi}$ is associated with the write in Lines 40 or 43, 
depending on whether $\ms{curr}$ is left or right child.
\item $\ms{curr}$ is a leaf with a ROUTING parent. Then $l_{\pi}$ is associated with the write in Lines 56 or 60, 
depending on whether $\ms{prev}$ is left or right child.
\end{enumerate}
For every $\pi = $\lit{delete}$(v)$ that returns $\false$, we have three cases:
\begin{enumerate}
\item If there exists a successful $\lit{delete}(v)$ whose linearization point lies in the interval of $\pi$,
then we take the first such $\lit{delete}(v)$ and linearize right after its linearization point.
\item If there exists successful $\lit{insert}(v)$ whose linearization point lies in the interval of $\pi$,
then we take the first such $\lit{insert}(v)$ and linearize right before its linearization point.
\item Otherwise, let $l_{\pi}$ be the call of $\pi$. 
\end{enumerate}

\textbf{Contains.}
For every $\pi = $\lit{contains}$(v)$ that returns $\true$, $l_{\pi}$ 
is associated with the read of state in Line 13 of Algorithm~\ref{alg:seq}.

For every $\pi = $\lit{contains}$(v)$ that returns $\false$, we have three cases that should be applied to the $\pi$ consequently:
\begin{enumerate}
\item If there exists successful $\lit{delete}(v)$ whose linearization points lies in the interval of $\pi$,
then we take the first such $\lit{delete}(v)$ and put $l_{\pi}$ right after its linearization point.
\item If there exists successful $\lit{insert}(v)$ which linearization points lies in the interval of $\pi$,
then we take the first such $\lit{insert}(v)$ and put $l_{\pi}$ right before its linearization point.
\item Otherwise, let $l_{\pi}$ be the call of $\pi$.
%\item The vertex with key $v$ was found in the tree. Then $l_{\pi}$ is associated with the read of state in Line 13.
%\item The vertex with key $v$ wasn't found in the tree. We have two cases. In the first case, if the linearization point of Then $l_{\pi}$ is associated with the last read of left or right children at Lines 16 and 18.
\end{enumerate}

To facilate the proof of correctness of the choice of linearization points, we need the following auxiliary theorem 
about the invariants on the structure of the binary search tree that must hold during the execution.

\begin{theorem}
\label{th:inv}
At any point of time, the algorithm preserves invariants on the structure of the binary search tree:
\begin{enumerate}
\item The root vertex always exists.
\item Every node with the state DATA or ROUTING is reachable from the root.
\item The binary search tree property is preserved, i.e., for any node $v$ the keys in its left subtree, 
if exists, are less than in $v$ and the keys in its right subtree, if exists, are bigger than in $v$.
\item Every ROUTING node has exactly 2 children.
\end{enumerate}
\end{theorem}
\begin{proof}
\textbf{Invariant 1.} The root is not null because key $+\infty$ in the root ensures that
we never call $\lit{delete}$ function with $+\infty$ as argument.

\textbf{Invariant 2.} We unlink the vertex, only if it has its state set to DELETED, 
in Lines 25, 40 or 43, 55 or 59, 56 or 60 of Algorithm~\ref{alg:concur-del}.

\textbf{Invariant 3.} We need to consider all possible cases of operations $\lit{insert}(v)$ and $\lit{delete}(v)$.
We prove this invariant by induction on the number of primitive operations, i.e., operations on base-objects.

Base case. 0 operations. The invariant is preserved because the tree contains only root with key $+\infty$.

Step $k \rightarrow k + 1$.
Note that we could consider only the primitive operations of the successful high-level operation, 
i.e, the operations that return $\true$, because unsuccessful ones do not change the structure of the tree.
For the same reason, we can consider only $\lit{insert}$ and $\lit{delete}$ operations.

Let the current operation be a primitive operation of successful $\pi = $\lit{insert}$(v)$ such that:
\begin{itemize}
\item There was a vertex with key $v$. Then the invariant was already preserved for that vertex before the $\pi$ call.
\item There was no vertex with key $v$. 
The invariant can break only for the operations in Lines 23 (25) of Algorithm~\ref{alg:concur-ins}.
But during these lines we have taken the lock in Line 19, so no other operation could change the state of $\ms{prev}$. 
Thus after Lines 23 (25) the invariant of $\ms{prev}$ holds and the invariant for the new vertex holds too.
\end{itemize}

Let the current operation be the primitive operation of successful $\pi = delete(v)$ such that:
\begin{itemize}
\item The vertex with key $v$ has two children. The structure of the tree is not changed, so the invariant is preserved.
\item The vertex has one child. 
The invariant can break only for primitive operations in Lines 28 (32) of Algorithm~\ref{alg:concur-del}. 
But there we take a lock on the corresponding link of $\ms{prev}$ in Lines 26 (30), 
so no other operation could make a structural change with $\ms{prev}$ because the same lock is required.
In Lines 28 (30) we relink the vertices from the same subtree of $\ms{prev}$. Thus the invariant is preserved.

\item The vertex is a leaf with a DATA parent. 
The the invariant can break only by primitive operations in Lines 41 (44). 
Again, as in the previous case, we take a lock on the corresponding link of $\ms{prev}$ in Lines 43 (47), 
so no other operation could perform structural change on $\ms{prev}$. Since we only delete the leaf, 
the invariant is preserved.
\item The vertex is a leaf with a ROUTING parent. 
Then the invariant can break only for the primitive operations in Lines 57 (61).
But we previously take locks at $\ms{prev}$ and $\ms{gprev}$ in Lines 47 (50), 32 and 52 (by call of validateAndTryLock function), 
so no other operation could perform structural changes on them. 
As a result of Lines 57 and 61, we relink the vertices in the same subtree of $\ms{gprev}$, thus the invariant is preserved.
\end{itemize}

\textbf{Invariant 4.} 
We set the state of vertex $v$ to ROUTING only if it has two children during $\lit{delete}(v)$ 
as witnessed in Line 18 of Algorithm~\ref{alg:concur-del}.
Consider an execution of $\pi = $\lit{delete}$(v)$ after taking the lock in Line 5. 
We should consider this line because only after taking the lock on the state we check the number of children.
The only operation that could change the number of children of $v$ is concurrent $\lit{delete}$ operation 
of a child $u$ which is a leaf.
But $\lit{delete}(u)$ takes the lock on the parent, i.e, vertex $v$, in Line 31 of Algorithm~\ref{alg:concur-del}. 
But this operation cannot be perfomed concurrently with $\pi$, hence, the invariant is maintained.
\end{proof}

\begin{theorem}{Linearizability}
\label{th:lin}
The algorithm is linearizable with respect to the set type.
\end{theorem}
\begin{proof}
TODO: recall what is S.
First we prove the linearizability of the subhistory with only successful $\lit{insert}$ and $\lit{delete}$ operations, 
because other operations do not affect the structure of the tree.
Then we prove the linearizability of the subhistory with only update operations, 
i.e., successful and unsuccessful $\lit{insert}(v)$ and $\lit{delete}(v)$.
And finally, we present the proof for the history with any type of operations.

\textbf{Successful update functions.}
Let $\tilde{S}_{succ}^k$ be the prefix of $\tilde{S}$ consisting of the first $k$ 
complete successful operations $\lit{insert}(v)$ or $\lit{delete}(v)$ with respect to their linearization points.
We prove by induction on $k$ that the sequence $\tilde{S}_{succ}^k$ is consistent with respect to the \emph{set} type.

The base case $k = 0$, i.e., there are no complete operations, is trivial.

Transition from $k$ to $k + 1$. Suppose that $\tilde{S}_{succ}^k$ is consistent with the \textit{set} type.
Let $\pi$ with argument $v \in \mathbb{Z}$ and its reponse $r_{\pi}$ be the last operation in $\tilde{S}_{succ}^{k + 1}$.
We want to prove that $\tilde{S}_{succ}^{k + 1}$ is consistent with $\pi$. For that, we check all possible types of $\pi$.

\begin{enumerate}
\item $\pi = $\lit{insert}$(v)$ that returns $\true$.

  By induction, it is enough to prove that there are no preceding operation with an argument $v$ 
  or the last preceding operation with an argument $v$ in $\tilde{S}_{succ}^{k + 1}$ is $\lit{delete}(v)$.
  We need to investigate two cases of insertion: whether $\pi$ finds the vertex with key $v$ in the tree or not.

  In the first case, $\pi$ finds a vertex with key $v$. Suppose the contrary. 
  Let the last preceding operation with an argument $v$ be $\pi' = insert(v)$.
  Suppose that $\pi'$ inserted a new vertex $w$. Because the linearization point of $\pi'$ precedes the linearization point of $\pi$ 
  and the linearization point of $\pi$ coincides with the read of the \textit{state} field, then $\pi$ gets to $w$. 
  By the same reason, the state of $w$, read at the linearization point of $\pi$, is DATA, 
  which is impossible because $\pi$ is successful.

  Thus, $\pi'$ found the existing vertex $w$ with key $v$.
  From the facts that the linearization point of $\pi'$ precedes the linearization point of $\pi$ and 
  that $\pi'$ and $\pi$ should take a write lock on the state of $w$ to perform an operation, it follows that
  $\pi$ could not change the state before $\pi'$ releases the lock. 
  But $\pi'$ released the lock only after it set the state of $w$ to DATA. 
  Thus, $\pi$ reads the state of $w$ as DATA and $\pi$ could not be successful.
  
  In the second case, $\pi$ does not find the vertex with key $v$. 
  Again, we suppose the opposite: the previous successful operation with $v$ is $\pi' = $\lit{insert}$(v)$.
  Since there is no vertex with key $v$, we want to take a lock at the corresponding link of the lowest unary node $p$ 
  found by the \textbf{traverse} function and then insert a new vertex. $\pi$ is successful,
  it inserts new vertex, but from the facts that the linearization point of $\pi'$ precedes the linearization point of $\pi$ 
  and that the location in the tree of the vertex with key $v$ is unique
  due to the Invariant 3 (Theorem~\ref{th:inv}), it follows that $\pi'$ has inserted new vertex 
  by taking a write lock on $p$ or has encountered existing vertex which was inserted by taking lock on the corresponding link of $p$. 
  Thus, by taking the lock on the corresponding link of $p$,
  $\pi$ encounters the existing vertex. 
  The change of pointer forces $\pi$ to restart the operation, getting to the first case and establishing the contradiction.

\item $\pi = $\lit{delete}$(v)$ that returns $\true$.

  By induction it is enough to prove that the preceding operation with 
  an argument $v$ in $\tilde{S}_{succ}^{k + 1}$ is $\lit{insert}(v)$.
  Suppose the opposite: let the last preceding operation with $v$ be 
  $\lit{delete}(v)$ or there is no preceding operation with an argument $v$. 
  If there is no such operation, then $\pi$ could not
  find a vertex with key $v$, because if other operation has inserted the vertex with key $v$ 
  before then its linearization point comes earlier. 
  Thus $\pi$ cannot successfully delete, which contradicts the result of $\pi$.
  Then the only remain possibility is that the previous successful operation is $\pi' = $\lit{delete}$(v)$. 
  Because $\pi$ is successful, it finds a vertex with key $v$. So, both $\pi$ and $\pi'$
  take locks on the state of the same vertex to perform an operation at linearization point.
  Because the linearization point of $\pi$ precedes the linearization point of $\pi'$, $\pi'$ has taken the lock earlier.
  $\pi$ finds the vertex with key $v$, therefore $\pi'$ could not unlink the vertex with key $v$.
  So, $\pi'$ has set the state of the vertex to ROUTING. When $\pi$ checks the state after obtaining the lock, 
  $\pi$ reads ROUTING and cannot delete the vertex. This contradicts the fact that $\pi$ is successful. 
\end{enumerate}

\textbf{Update operations.}
Let $\tilde{S}_m^k$ be the prefix of $\tilde{S}$ consisting of the first $k$ 
complete operations $\lit{insert}(v)$ or $\lit{delete}(v)$ 
with respect to their linearization points.
We prove by induction on $k$ that the sequence $\tilde{S}_m^k$ is consistent with respect to the \textit{set} type. 
We already proved that successful operations are consistent, then
we should prove that the linearization points of unsuccessful operations are consistent too.

The base case $k = 0$, i.e., there are no complete operations, is trivial.

Transition from $k$ to $k + 1$. Suppose that $\tilde{S}_{m}^k$ is consistent with the \textit{set} type.
Let $\pi$ with argument $v \in \mathbb{Z}$ and response $r_{\pi}$ be the last operation in $\tilde{S}_{m}^{k + 1}$.
We want to prove that $\tilde{S}_{m}^{k + 1}$ is consistent with $\pi$. For that, we check all the possible types of $\pi$.

If operation $k + 1$ is successful then it is consistent with the previous operations, because it is consistent with successful operations
and unsuccessful operations do not change the structure of the tree.

If the operation $k + 1$ is unsuccessful, we have two cases.
\begin{enumerate}
\item $\pi = $\lit{insert}$(v)$ that returns $\false$.

  By induction, it is enough to prove that the last preceding successful operation 
  with $v$ in $\tilde{S}^{k + 1}$ is $\lit{insert}(v)$.
  Suppose the opposite: let the last preceding successful operation with an argument $v$ 
  be $\lit{delete}(v)$ or there is no preceding operation with an argument $v$.
  If there is no such operation then $\pi$ could not find a vertex with key $v$,
  because if another operation has previously inserted the vertex, then its linearization point comes earlier. 
  Thus $\pi$ would successfully insert a new vertex with key $v$, which contradicts the result of $\pi$.
  Then the only remaining possibility is that the last preceding successful operation is $\pi' = $\lit{delete}$(v)$.
  Since $\pi$ returns $\false$, $\pi$ finds a vertex with key $v$.
  Both of $\pi$ and $\pi'$ take locks on the state of the vertex to perform an operation at their linearization points.
  The linearization point of $\pi'$ precedes the linearization point of $\pi$, then $\pi'$ has taken lock earlier. 
  $\pi$ finds the vertex with key $v$ then $\pi'$ cannot unlink the vertex with key $v$.
  So, $\pi'$ has set the state of the vertex to ROUTING. When $\pi$ checks the state after obtaining the lock,
  $\pi$ reads ROUTING and $\pi$ sets the state to DATA. This contradicts the fact that $\pi$ is unsuccessful.

\item $\pi = $\lit{delete}$(v)$ that returns $\false$.

  When we set the linearization point of $\pi$ relying on the successful operation in the interval of $\pi$, 
  the linearization point is correct: if we linearize right after successful 
  $\lit{delete}(v)$ then $\pi$ correctly returns $\false$;
  if we linearize right before successful $\pi' = $\lit{insert}$(v)$ 
  then by the proof of linearizability for successful operations 
  there exists preceding to $\pi'$ successful $\lit{delete}(v)$ or there are no successful operation 
  with an argument $v$ in $\tilde{S}$ before $\pi'$, thus $\pi$ correctly returns $\false$.

  So, it remains to consider the case when no successful operation were linearized in the interval of $\pi$.
  By induction, it is enough to prove that there is no preceding successful operation with $v$ or 
  the last preceding successful operation with $v$ in $\tilde{S_{m}}^{k + 1}$ is $\lit{delete}(v)$.
  Again, suppose the opposite: let the previous successful operation with $v$ be $\pi' = $\lit{insert}$(v)$.

  If $\pi'$ inserted new vertex, then $\pi$ reaches that vertex. 
  This is due to the fact that the linearization point of $\pi'$ is earlier than the call of $\pi$
  and, thus, the link to the new vertex existed before the call of $\pi$. 
  So, reaching the vertex, $\pi$ sees that the state is DATA.
  Which is impossible because $\pi$ is unsuccessful. So, $\pi'$ found the existing vertex $w$ with key $v$.
  From the fact that the linearization point of $\pi'$ precedes the start of $\pi$
  follows that $\pi$ reads the state after $\pi'$ changed it. 
  Thus $\pi$ reads from the state what $\pi'$ has written there, i.e. DATA.
  So, $\pi$ should remove the vertex with key $v$. This contradicts the fact that $\pi$ is unsuccessful.
\end{enumerate}

\textbf{All operations.}
And finally we prove correctness of the linearization points of all operations.

Let $\tilde{S}^k$ be the prefix of $\tilde{S}$ consisting of the first $k$ complete operations 
ordered by their linearization points.
We prove by induction on $k$ that the sequence $\tilde{S}^k$ is consistent with respect to the \emph{set} type. 
We already proved that update operations are consistent, then
we should prove that the linearization points of contains operations are consistent too.

The base case $k = 0$, i.e., there are no complete operations, is trivial.

Transition from $k$ to $k + 1$. Suppose that $\tilde{S}^k$ is consistent with the \emph{set} type.
Let $\pi$ with argument $v \in \mathbb{Z}$ and its reponse $r_{\pi}$ be the last operation in $\tilde{S}^{k + 1}$.
We want to proof, that $\tilde{S}^{k + 1}$ is consistent for the operation $\pi$. For that, we check all the possible types of $\pi$.

If the operation $k + 1$ is $\lit{insert}(v)$ and $\lit{delete}(v)$ 
then it is consistent with the previous $\lit{insert}(v)$ and $\lit{delete}(v)$ operations
while $\lit{contains}(v)$ operations do not change the structure of the tree.

If the operation is $\pi = $\lit{contains}$(v)$, we have two cases:
\begin{enumerate}
  \item $\pi$ returns $\true$.

  By induction, it is enough to prove that the last preceding successful operation 
  with $v$ in $\tilde{S}^{k + 1}$ is $\lit{insert}(v)$.
  Suppose the opposite: the last preceding successful operation with an argument $v$ 
  be $\lit{delete}(v)$ or there is no preceding successful operation with $v$.
  Operation $\pi$ gets to the vertex with key $v$. 
  If there were no successful operation with $v$ then there could not be a vertex with value $v$ in the tree.
  Now let the previous successful operation be $\pi' = $\lit{delete}$(v)$. 
  Due to the fact that the linearization point of $\pi'$ precedes the linearization point of $\pi$, it
  follows that $\pi'$ sets the state of the vertex $\pi$ to ROUTING or DELETED before $\pi$ reads it. 
  No other operation could change the state in between to DATA because 
  all primitive operations that set states to DATA are linearization points 
  of some operations and the linearization point of $\pi$ comes right after $\pi'$.
  Thus, $\pi$ reads the state as ROUTING or DELETED, which contradicts the fact that $\pi$ returns $\true$.

  \item $\pi$ returns $\false$.

  When we set the linearization point of $\pi$ relying on a successful update operation in the interval of $\pi$,
  then the linearization point is correct: 
  \begin{itemize}
    \item if we linearize right after successful $\lit{delete}(v)$, then $\pi$ correctly returns false;
    \item if we linearize right before successful $\pi' = $\lit{insert}$(v)$ then, 
    by the proof of linearizability on successful operations
    either there exists a preceding $\pi'$ successful $\lit{delete}(v)$ or 
    there exists no operation with an argument $v$ in $\tilde{S}$ before $\pi'$. 
    Thus $\pi$ correctly returns $\false$.
  \end{itemize}
  Thus, we are left with the case when no successful operation has its linearization point in the interval of $\pi$.
  By induction, it is enough to prove that there is no preceding successful operation with an argument $v$ 
  or the last preceding successful operation with an argument $v$ in $\tilde{S}^{k + 1}$ is $\lit{delete}(v)$.
  Again, suppose the opposite: the last preceding successful operation 
  with an argument $v$ is $\pi' = $\lit{insert}$(v)$.

  Suppose that $\pi'$ inserts a new vertex $w$. The linearization point of $\pi'$ precedes the start of the execution of $\pi$, 
  otherwise, the linearization point of $\pi'$ would lie in the interval of $\pi$.
  Therefore the link to the new vertex existed before the call of $\pi$. 
  So, $\pi$ reaches the vertex $w$ and sees that the \textit{state} field of $w$ is DATA.
  That contradicts the fact that $\pi$ is unsuccessful. Hence $\pi'$ finds the existing vertex $w$ with key $v$. 
  Because the linearization point of $\pi'$ precedes the start of the execution of $\pi$
  and the linearization point of $\pi'$ coincides with the primitive operation of assignmet set to DATA,
  it follows that $\pi$ reads the state of $w$ after $\pi'$ changed it to DATA. Thus $\pi$ reads DATA.
  So, $\pi$ could remove the vertex with key $v$. This contradicts the fact that $\pi$ is unsuccessful.
\end{enumerate}                                                      
\end{proof}

\subsection{Liveness. Deadlock-freedom}
\begin{theorem}{Deadlock-freedom}
The algorithm is deadlock-freedom.
\end{theorem}
\begin{proof}
  If thread executes $\pi=\lit{contains}(v)$, this thread always make progress, because $\lit{contains}$ is wait-free.
  
  Otherwise, take the top ``conflict'' node. Note if some thread $t_1$ failed to acquire a lock on this node it happens for two reasons:
  \begin{enumerate}
    \item There is another thread $t_2$ which hold a lock on this node. 
    Hence we acquire a lock from children to parent and hence this is the top node, this thread successfully acquires locks on higher nodes and
    makes progress.
    \item Some locking conditions are violated: it means between the traversal phase and attempting to acquire a lock some another thread
    $t_2$ changes expected condition. Thus thread $t_2$ has already made a progress.
  \end{enumerate}
\end{proof}

